SVGD: A Virtual Gradients Descent Method for Stochastic Optimization

Inspired by dynamic programming, we propose Stochastic Virtual Gradient Descent (SVGD) algorithm where the Virtual Gradient is defined by computational graph and automatic differentiation. The method is computationally efficient and has little memory requirements. We also analyze the theoretical convergence properties and implementation of the algorithm. Experimental results on multiple datasets and network models show that SVGD has advantages over other stochastic optimization methods.

==> alg-SVGD.tex <==
\begin{algorithm}[H]
	\DontPrintSemicolon
	\SetAlgoLined
	\SetNoFillComment
	\LinesNotNumbered
	
	\KwInput{$\boldsymbol{G}$: computational graph associated with function $J^{(\tau)} = L(\hat{y} (\boldsymbol{x}^{(\tau)}, \boldsymbol{\theta}), y^{(\tau)})$}
	\KwInput{$\alpha$: Learning rate}
	\KwInput{$m$: Minibatch size}
	\KwInput{$s \in [0, +\infty)$: Scaling coefficient}
	\KwInput{$\boldsymbol{\theta}$: Initial parameter}
	
	\tcc{define operator $\nabla^{(\boldsymbol{G}, \mathscr{T})}$ before training}
	\For{$\tilde{\boldsymbol{\sigma}}'_i \in \boldsymbol{V}_{\boldsymbol{\theta} \rightarrow \boldsymbol{\sigma}}^{\boldsymbol{G}} $}    
	{ 
		$\boldsymbol{r}_i = \boldsymbol{0}$ 
		\tcp*[l]{Initialize gradient accumulation variable}
		\For{$j \in \{ 1, \cdots, N_i \} $}
		{
			\eIf{$\tilde{\boldsymbol{f}}_i$ about $\tilde{\boldsymbol{\theta}}'_{i,j}$ is linear}
			{
				$\boldsymbol{g}_{\tilde{\boldsymbol{\theta}}'_{i,j} \rightarrow \tilde{\boldsymbol{\sigma}}'_i} (\mathscr{T}_{i,j} \nabla_{\tilde{\boldsymbol{\sigma}}'_i} J^{(\tau)}; \cdots; \cdots) 
				= \boldsymbol{g}_{\tilde{\boldsymbol{\theta}}'_{i,j} \rightarrow \tilde{\boldsymbol{\sigma}}'_i} (s \frac{\nabla_{\tilde{\boldsymbol{\sigma}}'_i} J^{(\tau)}}{\sqrt{\boldsymbol{r}_i + \epsilon}}; \cdots; \cdots)$ 
				\tcp*[l]{define $\mathscr{T}_{i,j}$}
			}{
				$\boldsymbol{g}_{\tilde{\boldsymbol{\theta}}'_{i,j} \rightarrow \tilde{\boldsymbol{\sigma}}'_i} (\mathscr{T}_{i,j} \nabla_{\tilde{\boldsymbol{\sigma}}'_i} J^{(\tau)}; \cdots; \cdots) 
				= \boldsymbol{g}_{\tilde{\boldsymbol{\theta}}'_{i,j} \rightarrow \tilde{\boldsymbol{\sigma}}'_i} (\nabla_{\tilde{\boldsymbol{\sigma}}'_i} J^{(\tau)}; \cdots; \cdots)$ 
				\tcp*[l]{define $\mathscr{T}_{i,j}$}
			}
		}
	}
	
	\tcc{update $\boldsymbol{\theta}$}
	\While{$\boldsymbol{V}_{\boldsymbol{\theta}^{(t)}}^{\boldsymbol{G}}$ not converged}
	{
		Sample a minibatch of $m$ examples from the training set $\{ \boldsymbol{x}^{(1)}, \cdots, \boldsymbol{x}^{(m)} \}$ with corresponding targets $y^{(i)}$. \\
		\For{$\tilde{\boldsymbol{\sigma}}'_i \in \boldsymbol{V}_{\boldsymbol{\theta} \rightarrow \boldsymbol{\sigma}}^{\boldsymbol{G}} $ parallel} 
		{
			$\boldsymbol{r}_i \leftarrow \rho \boldsymbol{r}_i + (1 - \rho) \frac{1}{m} \sum\limits_{i=\tau}^{m} \left( \nabla_{\tilde{\boldsymbol{\sigma}}'_i} J^{(\tau)}  \right)^2 $ 
			\tcp*[l]{Accumulate squared gradient}
		}
		\For{$\tilde{\boldsymbol{\theta}}_j \in \boldsymbol{V}_{\boldsymbol{\theta}}^{\boldsymbol{G}}$ parallel} 
		{
			$\tilde{\boldsymbol{\theta}}_j \leftarrow \tilde{\boldsymbol{\theta}}_j - \alpha \frac{1}{m} \sum\limits_{i=\tau}^{m} \nabla_{\tilde{\boldsymbol{\theta}}_j}^{(\boldsymbol{G}, \mathscr{T})} J^{(\tau)} $ 
			\tcp*[l]{apply update}
		}
	}
	
	\caption{\textit{SVGD}, our proposed algorithm for stochastic optimization. $(\nabla J)^2$ indicates the elementwise square $\nabla J \odot \nabla J$. Good default settings for the tested machine learning problems are $\epsilon = 10^{-6}$ and $\rho = 0.9$. All operations are element-wise.}
	\label{alg:SVGD}
\end{algorithm}
